Tropical bisectors and Voronoi diagrams

In this paper we initiate the study of tropical Voronoi diagrams. We start out with investigating bisectors of finitely many points with respect to arbitrary polyhedral norms. For this more general scenario we show that bisectors of three points are homeomorphic to a non-empty open subset of Euclidean space, provided that certain degenerate cases are excluded. Specializing our results to tropical bisectors then yields structural results and algorithms for tropical Voronoi diagrams.

==> beach_line.tex <==
\begin{figure}
  \begin{tikzpicture}[scale=0.6, x={(-0.95cm,-0.5cm)},y={(0.95cm,-0.5cm)}, z={(0cm,1cm)}]
    \scriptsize
    \clip (0, -4.5, -5.25) -- (0,-4.5,0.75) -- (0, 4.5, 5.25) -- (0,4.5, -0.75) --cycle;

    \draw (0,-0.3333, -1.5) -- (0,-1,-1.5) -- (0, -2, -2) -- (0,-1.5, -1) -- (0,-1.5, 0) -- (0,-1,1);

    \draw (0,-1,1) -- (0,-51, 51);
    \draw (0,-2,-2) -- (100, -2,-2);

    % sweepline
    \draw[dashed, thick] (0,1,102) -- (0,1,-98);

    % beachline
    \draw[ultra thick] (0, -1, 3) -- (0,1,3) -- (0,-1,1) -- (0,0,1) -- (0,0.5, 0.5) -- (0,0.5,0)-- (0,0,-1) -- (0,-0.3333, -1.5) -- (0,0,-2) -- (0,0,-3);
    \fill[color=sqsqsq,fill=sqsqsq,fill opacity=0.2] (0, -1, 3) -- (0,1,3) -- (0,-1,1) -- (0,0,1) -- (0,0.5, 0.5) -- (0,0.5,0)-- (0,0,-1) -- (0,-0.3333, -1.5) -- (0,0,-2) -- (0,0,-3) -- (0,4.5,-0.75) -- (0,4.5,5.25) -- cycle;

    \draw [thick, ->] (0,1.1,0.55) -- (0,1.5,0.75);
    \draw (0,1.3,0.65) node[anchor=north] {$v$};

    \draw[fill=white, draw=black] (0,0,0) circle (2.5pt);
    \draw (0,0,0) node[anchor=north east] {$(0,0,0)$};
    \draw[fill=white, draw=black] (0,1,3) circle (2.5pt);
    \draw (0,1,3) node[anchor=west] {$(0,1,3)$};
    \draw[fill=white, draw=black] (0,-3,-1) circle (2.5pt);
    \draw (0,-3,-1) node[anchor=north] {$(0,-3,-1)$};
    \draw[fill=white, draw=black] (0,-1,-3) circle (2.5pt);
    \draw (0,-1,-3) node[anchor=north east] {$(0,-1,-3)$};
    \draw[fill=white, draw=black] (0,2,-1) circle (2.5pt);
    \draw (0,2,-1) node[anchor=north] {$(0,2,-1)$};
  \end{tikzpicture}
  \hfill
  \begin{tikzpicture}[scale=0.6, x={(-0.95cm,-0.5cm)},y={(0.95cm,-0.5cm)}, z={(0cm,1cm)}]
    \scriptsize
    \clip (0, -4.5, -5.25) -- (0,-4.5,0.75) -- (0, 4.5, 5.25) -- (0,4.5, -0.75) --cycle;

    \draw (0, 0.3333,-1.3333) -- (0,0,-1.5) -- (0,-1,-1.5) -- (0, -2, -2) -- (0,-1.5, -1) -- (0,-1.5, 0) -- (0,-1,1) -- (0,0,1.5) -- (0,1,1.5) -- (0,1.25,1.625);

    \draw (0,1.5,0) -- (0,0.5, -1) -- (0, 0.3333, -1.3333);
    \draw (0,-1,1) -- (0,-51, 51);
    \draw (0,-2,-2) -- (100, -2,-2);
    \draw (0, 0.3333, -1.3333) -- (0, 0.5, -1.5) -- (0, 0.5, -2.25) -- (0, 1, -2.75) -- (0,1,-102.75);

    % sweepline
    \draw[dashed,thick] (0,3,102) -- (0,3,-98);

    % beachline
    \draw[ultra thick] (0,2,-2) -- (0,2.5,-1) -- (0,2.5,-0.5) -- (0,2,0) -- (0,1.5,0) -- (0,1.5,1.25) -- (0,1.25,1.625) -- (0,2,3) -- (0,2,4) -- (0,1,5) ;

    \fill[color=sqsqsq,fill=sqsqsq,fill opacity=0.2] (0,2,-2) -- (0,2.5,-1) -- (0,2.5,-0.5) -- (0,2,0) -- (0,1.5,0) -- (0,1.5,1.25) -- (0,1.25,1.625) -- (0,2,3) -- (0,2,4) -- (0,1,5) -- (0,4.5,5.25) -- (0,4.5,-0.75) -- cycle;

    \draw [thick, ->] (0,3.1,1.55) -- (0,3.5,1.75);
    \draw (0,3.3,1.65) node[anchor=north] {$v$};

    \draw[fill=white, draw=black] (0,0,0) circle (2.5pt);
    \draw (0,0,0) node[anchor=north] {$(0,0,0)$};
    \draw[fill=white, draw=black] (0,1,3) circle (2.5pt);
    \draw (0,1,3) node[anchor=north] {$(0,1,3)$};
    \draw[fill=white, draw=black] (0,-3,-1) circle (2.5pt);
    \draw (0,-3,-1) node[anchor=north] {$(0,-3,-1)$};
    \draw[fill=white, draw=black] (0,-1,-3) circle (2.5pt);
    \draw (0,-1,-3) node[anchor=north east] {$(0,-1,-3)$};
    \draw[fill=white, draw=black] (0,2,-1) circle (2.5pt);
    \draw (0,2,-1) node[anchor=north east] {$(0,2,-1)$};
  \end{tikzpicture}
  \caption{The beach line and the sweep line, for $t=1$ (left) and $t=3$ (right).}
  \label{fig:beachline}
\end{figure}

% Local Variables: 
% mode: latex
% mode: TeX-PDF
% TeX-master: "bisectors"
% mode: reftex
% mode: font-lock
% buffer-file-coding-system:utf-8-unix
% End: 


==> central_projection.tex <==
\begin{figure}\centering
  \begin{tikzpicture} [scale=1.2]
  \small

  \draw (0,0) circle (1cm);
  \draw (-0.866,0.5) arc (180:360:0.866 and 0.2);
  \draw[dashed] (0.866,0.5) arc (0:180:0.866 and 0.2);

  \draw (-2,-.5) circle (1cm);
  \draw (-2.866,0) arc (180:360:0.866 and 0.2);
  \draw[dashed] (0.866-2,0) arc (0:180:0.866 and 0.2);

  \draw (5,-.5) circle (1cm);
  \draw (-0.866+5,0) arc (180:360:0.866 and 0.2);
  \draw[dashed] (0.866+5,0) arc (0:180:0.866 and 0.2);

  \draw[dashed] (0,0) -- (1.5, 1.4);
  \draw[dashed](-2,-.5) -- (1.5, 1.4);
  \draw[dashed] (5,-.5) -- (1.5, 1.4);

  \draw[dashed] (0,0.5) -- (1.5, -.4);
  \draw[dashed](-2,0) -- (1.5, -.4);
  \draw[dashed] (5,0) -- (1.5, -.4);

  %points on the spheres
  \draw[fill=black] (-1.22, -0.08) circle(1pt);
  \draw[fill=black] (0.33, 0.32) circle(1pt);
  \draw[fill=black] (4.23,-0.085) circle(1pt);

  %circumcentres
  \draw[fill=black] (1.5,1.4) circle(1pt) node [anchor=south] {$p$};
  \draw[fill=black] (1.5, -.4) circle(1pt) node [anchor=north] {$r$};

  %three centers of spheres and circles
  \draw[fill=white, draw=black] (0,0) circle (2pt);
  \draw[fill=black] (0,0.5) circle (1pt);
  \draw(0,0) node[anchor=east] {$a_1$};

  \draw[fill=white, draw=black] (-2,-.5) circle (2pt);
  \draw[fill=black] (-2,0) circle (1pt);
  \draw(-2,-.5) node[anchor=north east] {$a_2$};

  \draw[fill=white, draw=black] (5, -.5) circle (2pt);
  \draw[fill=black] (5,0) circle (1pt);
  \draw(5,-.5) node[anchor=north west] {$a_3$};
  %\draw[dashed] (0,0 ) -- node[above]{$r$} (2,0);


  \end{tikzpicture}
  \caption{Construction of $\psi$ in the proof of Theorem~\ref{thm:3points} }
  \label{fig:central_projection}
\end{figure}

% Local Variables: 
% mode: latex
% mode: TeX-PDF
% TeX-master: "bisectors"
% mode: reftex
% mode: font-lock
% buffer-file-coding-system:utf-8-unix
% End: 


==> tvd.tex <==
\begin{figure}\centering
  \begin{tikzpicture}[scale=1, x={(-0.95cm,-0.5cm)},y={(0.95cm,-0.5cm)}, z={(0cm,1cm)}]
    \tikzset{tvd/.style = { very thick }}
    \tikzset{partition/.style = { dashed, opacity=0.3 }}
    \clip (0, -4.5, -5.25) -- (0,-4.5,0.75) -- (0, 4.5, 5.25) -- (0,4.5, -0.75) --cycle;

    \draw[tvd] (0,0,-1.5) -- (0,-1,-1.5) -- (0, -2, -2) -- (0,-1.5, -1) -- (0,-1.5, 0) -- (0,-1,1) -- (0,0,1.5) -- (0,1,1.5) -- (0,2,2) -- (0,3,2) -- (0,2,1) -- (0,1.5,0) -- (0,0.5, -1) -- (0, 0.3333, -1.3333) -- cycle;
    \draw[tvd] (0,-1,1) -- (0,-51, 51);
    \draw[tvd] (0,-2,-2) -- (100, -2,-2);
    \draw[tvd] (0,3,2) -- (0,103, 52);
    \draw[tvd] (0, 0.3333, -1.3333) -- (0, 0.5, -1.5) -- (0, 0.5, -2.25) -- (0, 1, -2.75) -- (0,1,-102.75);

    \draw[partition] (0,0,-100) -- (0,0,+100);
    \draw[partition] (0,-100,0) -- (0,+100, 0);
    \draw[partition] (-100,0,0) -- (100,0,0);

    \draw[partition] (0,1,3-100) -- (0,1,3+100);
    \draw[partition] (0,1-100,3) -- (0,1+100, 3);
    \draw[partition] (-100,1,3) -- (100,1,3);

    \draw[dashed, opacity=0.3] (0,-3,-100-1) -- (0,-3,+100-1);
    \draw[dashed, opacity=0.3] (-100,-3,-1) -- (100,-3,-1);

    \draw[dashed, opacity=0.3] (0,-1,-100-3) -- (0,-1,+100-3);
    \draw[dashed, opacity=0.3] (0,-100-1,-3) -- (0,+100-1, -3);
    \draw[dashed, opacity=0.3] (-100,0-1,-3) -- (100,-1,-3);

    \draw[dashed, opacity=0.3] (0,2,-100-1) -- (0,2,+100-1);
    \draw[dashed, opacity=0.3] (0,2-100,-1) -- (0,+100+2, -1);

    \draw (0,0,0) node[anchor=north, fill=white] {$(0,0,0)$};
    \draw[fill=white, draw=black] (0,0,0) circle (2.5pt);
    \draw (0,1,3) node[anchor=north, fill=white] {$(0,1.3)$};
    \draw[fill=white, draw=black] (0,1,3) circle (2.5pt);
    \draw (0,-3,-1) node[anchor=north, fill=white] {$(0,-3,-1)$};
    \draw[fill=white, draw=black] (0,-3,-1) circle (2.5pt);
    \draw (0,-1,-3) node[anchor=north, fill=white] {$(0,-1,-3)$};
    \draw[fill=white, draw=black] (0,-1,-3) circle (2.5pt);
    \draw (0,2,-1) node[anchor=north, fill=white] {$(0,2,-1)$};
    \draw[fill=white, draw=black] (0,2,-1) circle (2.5pt);
  \end{tikzpicture}
  \caption{Tropical Voronoi diagram of five points in $\torus{3}$. The decomposition of Voronoi regions into semi-polytropes is shown by dashed lines}
  \label{fig:tvd}
\end{figure}

% Local Variables: 
% mode: latex
% mode: TeX-PDF
% TeX-master: "bisectors"
% mode: reftex
% mode: font-lock
% buffer-file-coding-system:utf-8-unix
% End: 

